Cross Encoding as Augmentation: Towards Effective Educational Text Classification

Text classification in education, usually called auto-tagging, is the automated process of assigning relevant tags to educational content, such as questions and textbooks. However, auto-tagging suffers from a data scarcity problem, which stems from two major challenges: 1) it possesses a large tag space and 2) it is multi-label. Though a retrieval approach is reportedly good at low-resource scenarios, there have been fewer efforts to directly address the data scarcity problem. To mitigate these issues, here we propose a novel retrieval approach CEAA that provides effective learning in educational text classification. Our main contributions are as follows: 1) we leverage transfer learning from question-answering datasets, and 2) we propose a simple but effective data augmentation method introducing cross-encoder style texts to a bi-encoder architecture for more efficient inference. An extensive set of experiments shows that our proposed method is effective in multi-label scenarios and low-resource tags compared to state-of-the-art models.

==> tables/data_eda.tex <==
\begin{table*}[h]
    \caption{Dataset statistics for ARC, QC-Science, and EURLEX57K.}
    \label{tab:data_eda}
    \begin{tabular}{c c c c c c c}
        \toprule
\textbf{Dataset}      
& \textbf{Train }   
& \textbf{Dev }
& \textbf{Test}
& \textbf{Avg. context length }
& \textbf{\# of tags}
& \textbf{Avg \# of labels per context }
\\\midrule
ARC & 5579 & 778 & 1400 & 236 & 40 & 1 \\
QC-Science & 40895 & 2153 & 4784 & 32 & 312 & 1 \\
EURLEX57K & 45000 & 6000 & 6000 & 528 & 4271 & 5 \\
        \bottomrule
    \end{tabular}
\end{table*}

==> tables/few_data.tex <==
\begin{table*}[t]
    \caption{Eurlex Frequent Few Zero 실험 }
    \label{tab: few_data}
    \begin{tabular}{c c c c c c c}
        \toprule
\textbf{Methods}      
&\multicolumn{2}{c}{\textbf{Frequent}}  
&\multicolumn{2}{c}{\textbf{Few}}        
&\multicolumn{2}{c}{\textbf{Zero}}   


\\\midrule
ZERO-BIGRU-LWAN* & 0.764 & 0.780 & 0.561 & 0.510 & \textbf{0.438} & 0.345 \\
BERT & \textbf{0.835} & \textbf{0.846} & \textbf{0.686} & \textbf{0.636} & 0.028 & 0.023 \\
DPR & 0.748 & - & 0.673 & - & 0.393 & - \\
\ours & 0.781 & - & \textbf{0.686} & - & 0.427 & - \\
        \bottomrule
        
    \end{tabular}
\end{table*}

==> tables/multi_label.tex <==
% \begin{table}[h]

%     \begin{tabular}{c c c c c}
%         \toprule
% \multirow{2}{*}{\textbf{Methods}}
% &\multicolumn{2}{c}{\textbf{Single-label}}  
% &\multicolumn{2}{c}{\textbf{Multi-label}}\\
%  \cmidrule{2-5}
% &RP@5 & nDCG@5 & RP@5 & nDCG@5\\\hline
% BERT & - & -& 0.541 & 0.573 \\
% Bi-Encoder & 0.480 & 0.321 & - & - \\
% \ours & 0.506 & 0.339 & 0.559 & 0.578\\
%         \bottomrule
%     \end{tabular}
%     \caption{Multi-Label test}
%     \label{tab:multi_label}  
% \end{table}

==> tables/nDCG_arc.tex <==
\begin{table}[h]
    \begin{tabular}{c c c c}
        \toprule
\textbf{Methods}      
& \textbf{nDCG@1}   
& \textbf{nDCG@3}
& \textbf{nDCG@5}

\\\midrule
BERT & 0.527 & 0.640 & 0.670  \\
Bi-encoder & 0.539 & 0.651 & 0.679  \\
\ours & 0.559 & 0.662 & 0.686 \\
        \bottomrule
    \end{tabular}
    \caption{nDCG@K on ARC-Sciecne }
    \label{tab:nDCG_arc}    
\end{table}

==> tables/nDCG_qc.tex <==
\begin{table}[h]
    \begin{tabular}{c c c c}
        \toprule
\textbf{Methods}      
& \textbf{nDCG@1}   
& \textbf{nDCG@3}
& \textbf{nDCG@5}

\\\midrule
BERT & 0.688 & 0.796 & 0.813  \\
Bi-encoder & 0.694 & 0.796 & 0.811  \\
\ours & 0.702 & 0.798 & 0.814 \\
        \bottomrule
    \end{tabular}
    \caption{nDCG@K on QC-Sciecne }
    \label{tab:nDCG_QC}    
\end{table}

==> tables/qc_qual_result.tex <==

\begin{table*}[h]
    
    \caption{Comparison between Bi-encoder and Bi-encoder + \ours~on top-1 retrieved tag in which both tags were not ground truth of a given text. Bolded tag or tags are the most or equally relevant  related to the context. More examples are included in Appendix \ref{sec:appendix_qualitative}. }
    \label{tab: qual result}
    \small
    \begin{tabular}{l p{0.75\linewidth}}
    
    %\textbf{Context, Dataset Tag and Model Output}
    \\\toprule
    
    \textbf{Context} & \texttt{The sector in which employees have more job security is an organized sector.}
    \\
    \textbf{Ground Truth} & \texttt{social science >> economics >> sectors of the Indian economy }  
    \\
    \textbf{Bi-Encoder} & \texttt{social science >> civics : social and political life-i >> urban livelihoods}
    \\
    \textbf{Bi-Encoder + \ours}  &\texttt{\textbf{social science >> economics >> people as resource}}
    \\\hline
    \textbf{Context} & \texttt{Name the vitamin which helps in clotting of blood. Vitamin K }
    \\
    \textbf{Ground Truth} & \texttt{chemistry >> chemistry : part ii >> biomolecules}   
    \\
    \textbf{Bi-Encoder} & \texttt{\textbf{science >> components of food}}
    \\
    \textbf{Bi-Encoder + \ours} & \texttt{science >> life processes}
    \\\hline

    \textbf{Context} & \texttt{The type of climate in North-east India is wet. }
    \\
    \textbf{Ground Truth} & \texttt{science >> weather, climate and adaptations of animals to climate  }      
    \\
    \textbf{Bi-Encoder} & \texttt{\textbf{social science >> geography : the earth our habitat >> india : climate, vegetation and wildlife}}
    \\
    \textbf{Bi-Encoder + \ours} & \texttt{\textbf{social science >> geography: contemporary india - I >> climate}}
    \\\bottomrule
    \end{tabular}
\end{table*}


% \begin{table*}[t]
%     \caption{Comparison between Bi-encoder and \ours on top-1 retrieved tag in which was not gold label}
%     \label{tab: qual result}
%     \begin{tabular}{p{3.6cm} p{4cm} p{6.4cm}}
%         \toprule
% \textbf{Question text}      
% & \textbf{Ground truth}   
% & \textbf{Bi-encoder and \ours's top-1}
% \\\midrule
% The endemic species found in an area could be from any geographical unit.
% & science>>conservation of plants and animals     
% & political science>>political science : contemporary world politics>>environment and natural resources
% \\\cline{3-3}
% & & \textbf{social science>>geography : contemporary india - ii>>forest and wildlife resources}
% \\\hline

% The sector in which employees have more job security is an organized sector.
% & social science>>economics>>sectors of the Indian economy                        
% & social science>>civics : social and political life-i>>urban livelihoods
% \\\cline{3-3}
% & & \textbf{social science>>economics>>people as resource}
% \\\hline


% Name the vitamin which helps in clotting of blood. Vitamin K
% & chemistry>>chemistry : part ii>>biomolecules
% Underlying values       
% & \textbf{science>>components of food}
% \\\cline{3-3}
% & & science>>life processes
% \\\hline

% The type of climate in North-east India is wet.
% & science>>weather, climate and adaptations of animals to climate       
% & \textbf{social science>>geography : the earth our habitat>>india : climate, vegetation and wildlife}
% \\\cline{3-3}
% & & \textbf{social science>>geography: contemporary india - i>>climate}


% \\
%         \bottomrule
%     \end{tabular}
% \end{table*}
